Deblurring using Analysis-Synthesis Networks Pair

Blind image deblurring remains a challenging problem for modern artificial neural networks. Unlike other image restoration problems, deblurring networks fail behind the performance of existing deblurring algorithms in case of uniform and 3D blur models. This follows from the diverse and profound effect that the unknown blur-kernel has on the deblurring operator. We propose a new architecture which breaks the deblurring network into an analysis network which estimates the blur, and a synthesis network that uses this kernel to deblur the image. Unlike existing deblurring networks, this design allows us to explicitly incorporate the blur-kernel in the network's training. In addition, we introduce new cross-correlation layers that allow better blur estimations, as well as unique components that allow the estimate blur to control the action of the synthesis deblurring action. Evaluating the new approach over established benchmark datasets shows its ability to achieve state-of-the-art deblurring accuracy on various tests, as well as offer a major speedup in runtime.

==> ablation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Ablation study table %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]

\begin{tabular}{l|ccccc|ccccc}

\multirow{2}{*}{\textbf{Method}} &
\multicolumn{5}{ccccc|}{Synthesis + GT Kernels}  &
\multicolumn{5}{ccccc}{E2E} \\
%\cline{2-5}
 & \textbf{Blind} & \textbf{Additive guidance} & \textbf{Multiplicative guidance} & \textbf{Additive+Multiplicative guidance} & \textbf{Additive+Multiplicative guidance 1SGU} &
 \textbf{Random initialization} &
 \textbf{Pretaining before E2E training} &
 \textbf{Pretaining after E2E training} &
 \textbf{Multinet estimated kernel size } &
 \textbf{Multinet real kernel size } \\
\hline

\end{tabular}

\caption{}
\label{tab:kohler_numeric}
\end{table}
